Assessing Cyber-Physical Security in Industrial Control Systems

Over the last years, Industrial Control Systems (ICS) have become increasingly exposed to a wide range of cyber-physical threats. Efficient models and techniques able to capture their complex structure and identify critical cyber-physical components are therefore essential. AND/OR graphs have proven very useful in this context as they are able to semantically grasp intricate logical interdependencies among ICS components. However, identifying critical nodes in AND/OR graphs is an NP-complete problem. In addition, ICS settings normally involve various cyber and physical security measures that simultaneously protect multiple ICS components in overlapping manners, which makes this problem even harder. In this paper, we present an extended security metric based on AND/OR hypergraphs which efficiently identifies the set of critical ICS components and security measures that should be compromised, with minimum cost (effort) for an attacker, in order to disrupt the operation of vital ICS assets. Our approach relies on MAX-SAT techniques, which we have incorporated in META4ICS, a Java-based security metric analyser for ICS. We also provide a thorough performance evaluation that shows the feasibility of our method. Finally, we illustrate our methodology through a case study in which we analyse the security posture of a realistic Water Transport Network (WTN).

==> sections/analytical-evaluation-with-EPS.tex <==
\section{Performance evaluation}
\label{sec:analytical-exp}

We have performed a thorough experimental analysis that shows the feasibility and performance of our approach. In this section, we first describe the tool and methods used within the experiments. Afterwards, we explain the obtained results for independent security measures applied across the graph. Finally, we study the use of various security measures applied to multiple nodes simultaneously and the impact this overlapping poses in terms of computation time. The experimental evaluation has been performed using a MacBook Pro (15-inch, 2018), 2.9 GHz Intel Core i9, 32 GB 2400 MHz~DDR4. 

\subsection{Implementation prototype and AND/OR graph generation}

Our implementation prototype relies on \tool (\cite{BarrereSecMetric2019}), a Java-based security metric analyser for ICS, available at (\cite{BarrereMeta4icsGithub}). \tool consumes JSON specification files that describe ICS environments in the form of AND/OR graphs, and outputs their security score as well as the critical nodes that require utmost attention. In this work, we have extended \tool in order to cover hypergraph-related concepts and the application of multiple overlapping security measures over ICS network components.  

Within our experiments, we use synthetic pseudo-random AND/OR graphs of different size and composition that are generated as described in (\cite{BarrereSecMetric2019}). To create an AND/OR graph of size $n$, we first create the target node. Afterwards, we create a predecessor which has one of the three types (atomic, AND, OR) according to a probability given by a compositional configuration predefined for the experiment. For example, a configuration of $(60,20,20)$ means 60\% of atomic nodes, 20\% of AND nodes and 20\% of OR nodes. We repeat this process creating children on the respective nodes until we approximate the desired size of the graph~$n$. 

\subsection{Independent security measures}
Our first set of experiments studies the impact on scalability and performance when we increase the number of security measures applied independently on each network node. Figure~\ref{fig:exp1} shows the results of this evaluation over AND/OR graphs with up to 10000 nodes. 

\begin{figure}[!t]
	\centering
	\includegraphics[scale=0.65]{stats/scalability-conf-60-20-20.eps}
    \caption{Scalability evaluation while increasing graph size}
    \vspace{-0.3cm}
	\label{fig:exp1}
\end{figure}

We have measured the MAX-SAT resolution time for graphs of different sizes in four sub-experiments that use a different number of independent security controls (1, 5, 7 and 10) on each graph node. Each sub-experiment has been repeated 10 times and we have taken the average results. As expected, we can observe that the more security measures we use to protect each node independently, the more time is required to compute the underlying security metric. As explained in (\cite{BarrereSecMetric2019}), even when there are small time variations on each sub-experiment due to the compositional characteristics of some random AND/OR graphs, the overall behaviour remains relatively stable. 

Figure \ref{fig:exp2} shows a closer look at the logical transformation and MAX-SAT resolution times for graphs with 1000 nodes while increasing the use of independent security measures. We can observe that the MAX-SAT resolution time grows polynomially. This is essentially explained by the fact that each node variable $n$ is replaced by a larger disjunction with $x$ logical variables (for $x$ security measures) plus the node variable itself. Because each node is protected by a different set of security measures (no overlapping), such replacement just increments the size of the formula by a factor of $x$. Therefore, the overall process is still solved in polynomial time. In hypergraph terms, the smaller the hyperedges, the lower the computation time. 

\begin{figure}[t]
    \centering
    \includegraphics[scale=0.65]{stats/1x1-scalability-sec-measures.eps}
    \caption{Performance while increasing nodes' measures}
    \vspace{-0.3cm}
    \label{fig:exp2}
\end{figure}

The previous experiments are focused on security measures that are applied individually on each ICS component. As mentioned before, however, many security measures may be used to protect two or more components altogether in practice, e.g. fenced areas. In the next section, we evaluate our approach considering multiple overlapping security measures. 


\subsection{Overlapping security measures}

In order to analyse scenarios where two or more nodes may be protected by the same security control, we use a simple probabilistic method to generate a protection assignment as follows. Let $x$ be the number of security measures to be applied on each graph node $n \in V_{AT}$. We then traverse the set $V_{AT}$, and for each node, we stochastically choose whether to assign the same security measure used with the last node, or conversely, to use a new one. In mathematical terms, we apply the same security control with probability $p$ (positive overlapping), or we apply a new one with probability $1-p$ (no overlapping).  
We repeat the above procedure $x$ times. Figure~\ref{fig:exp3} shows the behaviour of the MAX-SAT resolution time over graphs with 1000 nodes that have been protected following the previous assignment. 

\begin{figure}[!t]
    \centering
    \includegraphics[scale=0.65]{stats/overlapping-variation-n1000-m10-v2.eps}
    \caption{Variation analysis of overlapping measures}
    \vspace{-0.3cm}
    \label{fig:exp3}
\end{figure}

\begin{figure}[!b]
    \centering
    \includegraphics[scale=0.65]{stats/stacked-x1000.eps}
    \caption{Overlapping analysis on graphs of different sizes}
    \vspace{-0.3cm}
    \label{fig:exp4}
\end{figure}

We can observe that, as the probability of overlapping increases from 0 to 1, the MAX-SAT resolution time decreases. In other words, the greater the level of overlapping, the easier is for the MAX-SAT solver engine to find the solution. In addition, this behaviour is observed independently of the number of security measures applied in the experiment. In logical terms, this happens because a security measure that protects many nodes will appear on the logical expansion of all of them (step~2, Section~\ref{sec:problem-spec}), and therefore, the MAX-SAT solver leverages such interdependency to speed up the overall resolution process. We have performed a similar analysis on larger AND/OR graphs and the results indicate the same behavioural pattern, as shown in Figure~\ref{fig:exp4}. 

The experiments involve AND/OR graphs with 1000 to 10000 nodes, using 5 security measures on each node. 
As expected, the results suggest that the more nodes are protected by the same security measures (i.e. higher probability), the faster is the resolution process. In the next section, we validate our approach through a comprehensive case study. 

